MedNNS: Supernet-based Medical Task-Adaptive Neural Network Search

Deep learning (DL) has achieved remarkable progress in the field of medical imaging. However, adapting DL models to medical tasks remains a significant challenge, primarily due to two key factors: (1) architecture selection, as different tasks necessitate specialized model designs, and (2) weight initialization, which directly impacts the convergence speed and final performance of the models. Although transfer learning from ImageNet is a widely adopted strategy, its effectiveness is constrained by the substantial differences between natural and medical images. To address these challenges, we introduce Medical Neural Network Search (MedNNS), the first Neural Network Search framework for medical imaging applications. MedNNS jointly optimizes architecture selection and weight initialization by constructing a meta-space that encodes datasets and models based on how well they perform together. We build this space using a Supernetwork-based approach, expanding the model zoo size by 51x times over previous state-of-the-art (SOTA) methods. Moreover, we introduce rank loss and Fr\'echet Inception Distance (FID) loss into the construction of the space to capture inter-model and inter-dataset relationships, thereby achieving more accurate alignment in the meta-space. Experimental results across multiple datasets demonstrate that MedNNS significantly outperforms both ImageNet pre-trained DL models and SOTA Neural Architecture Search (NAS) methods, achieving an average accuracy improvement of 1.7% across datasets while converging substantially faster. The code and the processed meta-space is available at https://github.com/BioMedIA-MBZUAI/MedNNS.

==> arxiv_version_copy.tex <==
@inproceedings{deng2009imagenet,
  title={Imagenet: A large-scale hierarchical image database},
  author={Deng, Jia and Dong, Wei and Socher, Richard and Li, Li-Jia and Li, Kai and Fei-Fei, Li},
  booktitle={2009 IEEE conference on computer vision and pattern recognition},
  pages={248--255},
  year={2009},
  organization={Ieee}
}
@article{zhuang2020transferlearning,
  title={A comprehensive survey on transfer learning},
  author={Zhuang, Fuzhen and Qi, Zhiyuan and Duan, Keyu and Xi, Dongbo and Zhu, Yongchun and Zhu, Hengshu and Xiong, Hui and He, Qing},
  journal={Proceedings of the IEEE},
  volume={109},
  number={1},
  pages={43--76},
  year={2020},
  publisher={Ieee}
}
@article{prevedello2019challenges,
  title={Challenges related to artificial intelligence research in medical imaging and the importance of image analysis competitions},
  author={Prevedello, Luciano M and Halabi, Safwan S and Shih, George and Wu, Carol C and Kohli, Marc D and Chokshi, Falgun H and Erickson, Bradley J and Kalpathy-Cramer, Jayashree and Andriole, Katherine P and Flanders, Adam E},
  journal={Radiology: Artificial Intelligence},
  volume={1},
  number={1},
  pages={e180031},
  year={2019},
  publisher={Radiological Society of North America}
}
@article{raghu2019transfusion,
  title={Transfusion: Understanding transfer learning for medical imaging},
  author={Raghu, Maithra and Zhang, Chiyuan and Kleinberg, Jon and Bengio, Samy},
  journal={Advances in neural information processing systems},
  volume={32},
  year={2019}
}
@article{kim2022transfer,
  title={Transfer learning for medical image classification: a literature review},
  author={Kim, Hee E and Cosa-Linan, Alejandro and Santhanam, Nandhini and Jannesari, Mahboubeh and Maros, Mate E and Ganslandt, Thomas},
  journal={BMC medical imaging},
  volume={22},
  number={1},
  pages={69},
  year={2022},
  publisher={Springer}
}

@article{godasu2020transfer,
  title={Transfer learning in medical image classification: Challenges and opportunities},
  author={Godasu, Rajesh and Zeng, David and Sutrave, Kruttika},
  journal={Transfer},
  volume={5},
  pages={28--2020},
  year={2020}
}
@article{yu2021frechet,
  title={Frechet inception distance (fid) for evaluating gans},
  author={Yu, Yu and Zhang, Weibin and Deng, Yun},
  journal={China University of Mining Technology Beijing Graduate School},
  volume={3},
  year={2021}
}
@article{yang2023medmnist,
  title={Medmnist v2-a large-scale lightweight benchmark for 2d and 3d biomedical image classification},
  author={Yang, Jiancheng and Shi, Rui and Wei, Donglai and Liu, Zequan and Zhao, Lin and Ke, Bilian and Pfister, Hanspeter and Ni, Bingbing},
  journal={Scientific Data},
  volume={10},
  number={1},
  pages={41},
  year={2023},
  publisher={Nature Publishing Group UK London}
}
@article{zhang2021tumor,
  title={Tumor detection using deep learning method in automated breast ultrasound},
  author={Zhang, Zilu and Li, Yanfeng and Wu, Wen and Chen, Houjin and Cheng, Lin and Wang, Shu},
  journal={Biomedical signal processing and control},
  volume={68},
  pages={102677},
  year={2021},
  publisher={Elsevier}
}
@article{liu2024towards,
  title={Towards more precise automatic analysis: a systematic review of deep learning-based multi-organ segmentation},
  author={Liu, Xiaoyu and Qu, Linhao and Xie, Ziyue and Zhao, Jiayue and Shi, Yonghong and Song, Zhijian},
  journal={BioMedical Engineering OnLine},
  volume={23},
  number={1},
  pages={52},
  year={2024},
  publisher={Springer}
}
@article{qureshi2019recent,
  title={Recent development on detection methods for the diagnosis of diabetic retinopathy},
  author={Qureshi, Imran and Ma, Jun and Abbas, Qaisar},
  journal={Symmetry},
  volume={11},
  number={6},
  pages={749},
  year={2019},
  publisher={MDPI}
}
@article{boulila2024effective,
  title={An effective weight initialization method for deep learning: Application to satellite image classification},
  author={Boulila, Wadii and Alshanqiti, Eman and Alzahem, Ayyub and Koubaa, Anis and Mlaiki, Nabil},
  journal={Expert Systems with Applications},
  pages={124344},
  year={2024},
  publisher={Elsevier}
}
@inproceedings{skorski2021revisiting,
  title={Revisiting weight initialization of deep neural networks},
  author={Skorski, Maciej and Temperoni, Alessandro and Theobald, Martin},
  booktitle={Asian Conference on Machine Learning},
  pages={1192--1207},
  year={2021},
  organization={PMLR}
}
@inproceedings{he2016deep,
  title={Deep residual learning for image recognition},
  author={He, Kaiming and Zhang, Xiangyu and Ren, Shaoqing and Sun, Jian},
  booktitle={Proceedings of the IEEE conference on computer vision and pattern recognition},
  pages={770--778},
  year={2016}
}
@article{elsken2019neural,
  title={Neural architecture search: A survey},
  author={Elsken, Thomas and Metzen, Jan Hendrik and Hutter, Frank},
  journal={Journal of Machine Learning Research},
  volume={20},
  number={55},
  pages={1--21},
  year={2019}
}
@article{wang2024mednas,
  title={Mednas: Multiscale training-free neural architecture search for medical image analysis},
  author={Wang, Yan and Zhen, Liangli and Zhang, Jianwei and Li, Miqing and Zhang, Lei and Wang, Zizhou and Feng, Yangqin and Xue, Yu and Wang, Xiao and Chen, Zheng and others},
  journal={IEEE Transactions on Evolutionary Computation},
  volume={28},
  number={3},
  pages={668--681},
  year={2024},
  publisher={IEEE}
}
@article{white2023neural,
  title={Neural architecture search: Insights from 1000 papers},
  author={White, Colin and Safari, Mahmoud and Sukthanker, Rhea and Ru, Binxin and Elsken, Thomas and Zela, Arber and Dey, Debadeepta and Hutter, Frank},
  journal={arXiv preprint arXiv:2301.08727},
  year={2023}
}
@article{cai2019once,
  title={Once-for-all: Train one network and specialize it for efficient deployment},
  author={Cai, Han and Gan, Chuang and Wang, Tianzhe and Zhang, Zhekai and Han, Song},
  journal={arXiv preprint arXiv:1908.09791},
  year={2019}
}
@inproceedings{mecharbat2023hyt,
  title={Hyt-nas: Hybrid transformers neural architecture search for edge devices},
  author={Mecharbat, Lotfi Abdelkrim and Benmeziane, Hadjer and Ouarnoughi, Hamza and Niar, Smail},
  booktitle={Proceedings of the 2023 Workshop on Compilers, Deployment, and Tooling for Edge AI},
  pages={41--45},
  year={2023}
}
@article{jeong2021task,
  title={Task-adaptive neural network search with meta-contrastive learning},
  author={Jeong, Wonyong and Lee, Hayeon and Park, Geon and Hyung, Eunyoung and Baek, Jinheon and Hwang, Sung Ju},
  journal={Advances in Neural Information Processing Systems},
  volume={34},
  pages={21310--21324},
  year={2021}
}
@inproceedings{benmeziane2024medical,
  title={Medical neural architecture search: Survey and taxonomy},
  author={Benmeziane, Hadjer and Hamzaoui, Imane and Cherif, Zayneb and El Maghraoui, Kaoutar},
  booktitle={International Joint Conference on Artificial Intelligence},
  year={2024}
}
@article{koonce2021mobilenetv3,
  title={MobileNetV3},
  author={Koonce, Brett and Koonce, Brett},
  journal={Convolutional Neural Networks with Swift for Tensorflow: Image Recognition and Dataset Categorization},
  pages={125--144},
  year={2021},
  publisher={Springer}
}
@inproceedings{tan2019mnasnet,
  title={Mnasnet: Platform-aware neural architecture search for mobile},
  author={Tan, Mingxing and Chen, Bo and Pang, Ruoming and Vasudevan, Vijay and Sandler, Mark and Howard, Andrew and Le, Quoc V},
  booktitle={Proceedings of the IEEE/CVF conference on computer vision and pattern recognition},
  pages={2820--2828},
  year={2019}
}
@inproceedings{liu2018progressive,
  title={Progressive neural architecture search},
  author={Liu, Chenxi and Zoph, Barret and Neumann, Maxim and Shlens, Jonathon and Hua, Wei and Li, Li-Jia and Fei-Fei, Li and Yuille, Alan and Huang, Jonathan and Murphy, Kevin},
  booktitle={Proceedings of the European conference on computer vision (ECCV)},
  pages={19--34},
  year={2018}
}
@article{cai2018proxylessnas,
  title={Proxylessnas: Direct neural architecture search on target task and hardware},
  author={Cai, Han and Zhu, Ligeng and Han, Song},
  journal={arXiv preprint arXiv:1812.00332},
  year={2018}
}
@inproceedings{nayman2021hardcore,
  title={Hardcore-nas: Hard constrained differentiable neural architecture search},
  author={Nayman, Niv and Aflalo, Yonathan and Noy, Asaf and Zelnik, Lihi},
  booktitle={International Conference on Machine Learning},
  pages={7979--7990},
  year={2021},
  organization={PMLR}
}
@inproceedings{huang2017densely,
  title={Densely connected convolutional networks},
  author={Huang, Gao and Liu, Zhuang and Van Der Maaten, Laurens and Weinberger, Kilian Q},
  booktitle={Proceedings of the IEEE conference on computer vision and pattern recognition},
  pages={4700--4708},
  year={2017}
}
@inproceedings{tan2019efficientnet,
  title={Efficientnet: Rethinking model scaling for convolutional neural networks},
  author={Tan, Mingxing and Le, Quoc},
  booktitle={International conference on machine learning},
  pages={6105--6114},
  year={2019},
  organization={PMLR}
}
@inproceedings{zoph2018learning,
  title={Learning transferable architectures for scalable image recognition},
  author={Zoph, Barret and Vasudevan, Vijay and Shlens, Jonathon and Le, Quoc V},
  booktitle={Proceedings of the IEEE conference on computer vision and pattern recognition},
  pages={8697--8710},
  year={2018}
}
@inproceedings{matsoukas2022makes,
  title={What makes transfer learning work for medical images: Feature reuse \& other factors},
  author={Matsoukas, Christos and Haslum, Johan Fredin and Sorkhei, Moein and S{\"o}derberg, Magnus and Smith, Kevin},
  booktitle={Proceedings of the IEEE/CVF Conference on Computer Vision and Pattern Recognition},
  pages={9225--9234},
  year={2022}
}
@inproceedings{pattnayak2024automated,
  title={Automated Skin Lesion Analysis and Classification Using AI},
  author={Pattnayak, Parthasarathi and Patnaik, Sanghamitra and Patra, Sudhansu Shekhar and Gourisaria, Mahendra Kumar and Singh, Satyendr and Barik, Lalbihari},
  booktitle={2024 4th International Conference on Sustainable Expert Systems (ICSES)},
  pages={1491--1498},
  year={2024},
  organization={IEEE}
}
@article{kouli2022automated,
  title={Automated brain tumor identification using magnetic resonance imaging: A systematic review and meta-analysis},
  author={Kouli, Omar and Hassane, Ahmed and Badran, Dania and Kouli, Tasnim and Hossain-Ibrahim, Kismet and Steele, J Douglas},
  journal={Neuro-oncology advances},
  volume={4},
  number={1},
  pages={vdac081},
  year={2022},
  publisher={Oxford University Press US}
}
@inproceedings{chu2021fairnas,
  title={Fairnas: Rethinking evaluation fairness of weight sharing neural architecture search},
  author={Chu, Xiangxiang and Zhang, Bo and Xu, Ruijun},
  booktitle={Proceedings of the IEEE/CVF International Conference on computer vision},
  pages={12239--12248},
  year={2021}
}
@article{kingma2014adam,
  title={Adam: A method for stochastic optimization},
  author={Kingma, Diederik P and Ba, Jimmy},
  journal={arXiv preprint arXiv:1412.6980},
  year={2014}
}

==> sections/4.Ablation.tex <==












==> sections/draft.tex <==

\begin{table}[ht]
    \centering
    \begin{adjustbox}{max width=1\textwidth}
    \begin{tabular}{@{}lcccccc@{}}
        \toprule
        \textbf{Method}    & \textbf{Pneumonia} & \textbf{OrganS} & \textbf{Tissue} & \textbf{Derma} & \textbf{Blood} & \textbf{Breast}  \\ 
        \midrule
        \multicolumn{8}{l}{\textbf{Models}} \\ 
        MobileNetV3   & 90.22\% & 67.63\% & -   & $\pm$   &  88.34\% &  85.89\%\\ 
        EfficientNet_{B0}  & 91.99\% & 76.95\% & -   & 76.36\%   & 87.31\% & 83.33\%  \\ 
        EfficientNet_{B4}  & 92.31\% & 81.14\%  &      & 74.41\%  & 96.20\%  &   \\ 
        ResNet18      & 86.51\% & 77.64\% & -   & 75.16\% &  96.17\% &  89.74\% \\ 
        ResNet50      & 85.91\% & 77.86\% & 63.12\%   & 73.56\% &  & 89.10\%  \\ 
        DenseNet121   & 93.27\% & 69.15\% & 68.12\%  & 75.86\% & 96.38\%  &  89.10\%\\ 
        \midrule
        \multicolumn{8}{l}{\textbf{NAS methods}} \\ 
        ProxylessNAS  & 94.07\%     & 81.12\%   & 68.60\%  & 76.11\%  &  96.43\% & 89.74\% \\ 
        MNASNet       & 89.90\% & 79.84\% & \textbf{69.63\%}  &  75.46\% & 96.25\% & 87.82\% \\  
        NASNet        & 94.87\%       & 80.73\%      & 68.54\%  & 74.86\%  & 96.05\% &  90.38\% \\ 
        OFA           & -       & -       & -   &    &  &  \\ 
        \midrule
        \multicolumn{8}{l}{\textbf{MedNNS (ours)}} \\ 
        MedNNS_{T1}            & 94.39\% & \textbf{81.53\%} & 
        68.93\%
        &  \textbf{79.70\%} & \textbf{96.93\%}  & \textbf{92.31\%} \\ 
        MedNNS_{T5}            & \textbf{96.15\%} & \textbf{82.10\%} & 
        69.13\%
        & \textbf{79.70\%} & \textbf{97.46\%} & \textbf{92.31\%} \\ 
        MedNNS_{T10}           & \textbf{96.15\%} & \textbf{82.34\%} & 
        69.18\%
        & \textbf{79.70\%} & \textbf{97.46\%} & \textbf{92.31\%}  \\ 
        \bottomrule
    \end{tabular}
    \end{adjustbox}
    \caption{Comparison of Methods Across Datasets}
    \label{tab:comparison}
\end{table}

\begin{table}[ht]
\centering
\small
\begin{adjustbox}{max width=1.2\textwidth}
\begin{tabular}{@{}lcccccc@{}}
\toprule
\textbf{Method} & \multicolumn{1}{c}{\textbf{Pneumonia}} & \multicolumn{1}{c}{\textbf{OrganS}} & \multicolumn{1}{c}{\textbf{Tissue}} & \multicolumn{1}{c}{\textbf{Derma}} & \multicolumn{1}{c}{\textbf{Blood}} & \multicolumn{1}{c}{\textbf{Breast}} \\ 
\cmidrule(lr){2-7}
                & Ep1/Ep10/Ep50/Ep100 & Ep1/Ep10/Ep50/Ep100 & Ep1/Ep10/Ep50/Ep100 & Ep1/Ep10/Ep50/Ep100 & Ep1/Ep10/Ep50/Ep100 & Ep1/Ep10/Ep50/Ep100 \\ 
\midrule
\multicolumn{7}{l}{\textbf{Models}} \\ 
MobileNetV3        & - / - / - / 90.22\%   & - / - / - / 67.63\%   & - / - / - / -       & - / - / - / $\pm$   & - / - / - / 88.34\%   & - / - / - / 85.89\%  \\[0.5ex]
EfficientNet\textsubscript{B0} & - / - / - / 91.99\%   & - / - / - / 76.95\%   & - / - / - / -       & - / - / - / 76.36\%  & - / - / - / 87.31\%   & - / - / - / 83.33\%  \\[0.5ex]
EfficientNet\textsubscript{B4} & - / - / - / 92.31\%   & - / - / - / 81.14\%   & - / - / - / -       & - / - / - / 74.41\%  & - / - / - / 96.20\%   & - / - / - / -        \\[0.5ex]
ResNet18           & - / - / - / 86.51\%   & - / - / - / 77.64\%   & - / - / - / -       & - / - / - / 75.16\%  & - / - / - / 96.17\%   & - / - / - / 89.74\%  \\[0.5ex]
ResNet50           & - / - / - / 85.91\%   & - / - / - / 77.86\%   & - / - / - / 63.12\%  & - / - / - / 73.56\%  & - / - / - / -        & - / - / - / 89.10\%  \\[0.5ex]
DenseNet121        & - / - / - / 93.27\%   & - / - / - / 69.15\%   & - / - / - / 68.12\%  & - / - / - / 75.86\%  & - / - / - / 96.38\%   & - / - / - / 89.10\%  \\[1ex]
\multicolumn{7}{l}{\textbf{NAS methods}} \\ 
ProxylessNAS       & - / - / - / 94.07\%   & - / - / - / 81.12\%   & - / - / - / 68.60\%  & - / - / - / 76.11\%  & - / - / - / 96.43\%   & - / - / - / 89.74\%  \\[0.5ex]
MNASNet            & - / - / - / 89.90\%   & - / - / - / 79.84\%   & - / - / - / \textbf{69.63\%} & - / - / - / 75.46\%  & - / - / - / 96.25\%   & - / - / - / 87.82\%  \\[0.5ex]
NASNet             & - / - / - / 94.87\%   & - / - / - / 80.73\%   & - / - / - / 68.54\%  & - / - / - / 74.86\%  & - / - / - / 96.05\%   & - / - / - / 90.38\%  \\[0.5ex]
OFA                & - / - / - / -         & - / - / - / -         & - / - / - / -        & - / - / - / -        & - / - / - / -         & - / - / - / -        \\[1ex]
\multicolumn{7}{l}{\textbf{MedNNS (ours)}} \\ 
MedNNS\textsubscript{T1}  & 85.0/90.0/93.0/94.3\%  & 75.00/78.00/80.00/81.53 & 65.00/67.00/68.50/68.93  & 70.00/75.00/78.00/79.70  & 90.00/94.00/96.00/96.93  & 80.00/85.00/90.00/92.31  \\[0.5ex]
MedNNS\textsubscript{T5}  & 86.00/92.00/95.00/96.15  & 76.00/80.00/81.00/82.10 & 66.00/68.00/69.00/69.13  & 72.00/77.00/79.00/79.70  & 91.00/95.00/97.00/97.46  & 82.00/87.00/90.00/92.31  \\[0.5ex]
MedNNS\textsubscript{T10} & 86.50/92.50/95.50/96.15  & 76.50/80.50/81.20/82.34  & 66.5/68.5/69.1/69.2\%  & 72.5/77.5/79.5/79.7\%  & 91.50/95.50/97.50/97.46\%  & 82.50/87.50/90.50/92.31\%  \\
\bottomrule
\end{tabular}
\end{adjustbox}
\caption{Comparison of Methods Across Datasets with Test Accuracies at Epochs 1/10/50/100. A “–” indicates that data for that epoch is not available.}
\label{tab:comparison_epochs}
\end{table}

\begin{table}[ht]
\centering
\renewcommand{\arraystretch}{1.2}
\begin{adjustbox}{max width=\textwidth}
\begin{tabular}{|l|c|c|c|c|c|c|}
\hline
\textbf{Method} 
  & \textbf{Pneumonia} 
  & \textbf{OrganS} 
  & \textbf{Tissue} 
  & \textbf{Derma} 
  & \textbf{Blood} 
  & \textbf{Breast} \\
\hline
\multicolumn{7}{|c|}{Test Accuracies: Epoch 1 \, | \, Epoch 10 \, | \, Epoch 100} \\
\hline
\multicolumn{7}{|l|}{\textbf{Models}} \\
\hline
MobileNetV3 
  & \begin{tabular}{c|c|c} 85.6\% & 88.5\% & 92.8\% \end{tabular}
  & \begin{tabular}{c|c|c} - & - & - \end{tabular}
  & \begin{tabular}{c|c|c} - & - & - \end{tabular}
  & \begin{tabular}{c|c|c} - & - & - \end{tabular}
  & \begin{tabular}{c|c|c} - & - & - \end{tabular}
  & \begin{tabular}{c|c|c} - & - & - \end{tabular} \\
\hline
EfficientNet\textsubscript{B0} 
  & \begin{tabular}{c|c|c} 64.4\% & 85.6\% & 92.3\% \end{tabular}
  & \begin{tabular}{c|c|c} 55.3\% & 78.1\% & 81.2\% \end{tabular}
  & \begin{tabular}{c|c|c} - & - & - \end{tabular}
  & \begin{tabular}{c|c|c} - & - & - \end{tabular}
  & \begin{tabular}{c|c|c} - & - & - \end{tabular}
  & \begin{tabular}{c|c|c} - & - & - \end{tabular} \\
\hline
EfficientNet\textsubscript{B4} 
  & \begin{tabular}{c|c|c} 73.1\% & 85.6\% & 92.0\% \end{tabular}
  & \begin{tabular}{c|c|c} 42.2\% & 74.5\% & 81.1\% \end{tabular}
  & \begin{tabular}{c|c|c} - & - & - \end{tabular}
  & \begin{tabular}{c|c|c} - & - & - \end{tabular}
  & \begin{tabular}{c|c|c} - & - & - \end{tabular}
  & \begin{tabular}{c|c|c} - & - & - \end{tabular} \\
\hline
ResNet18 
  & \begin{tabular}{c|c|c} 89.1\% & 93.1\% & 95.2\% \end{tabular}
  & \begin{tabular}{c|c|c} 60.4\% & 66.5\% & 80.6\% \end{tabular}
  & \begin{tabular}{c|c|c} - & - & - \end{tabular}
  & \begin{tabular}{c|c|c} - & - & - \end{tabular}
  & \begin{tabular}{c|c|c} - & - & - \end{tabular}
  & \begin{tabular}{c|c|c} - & - & - \end{tabular} \\
\hline
ResNet50 
  & \begin{tabular}{c|c|c} 81.7\% & 91.3\% & 93.9\% \end{tabular}
  & \begin{tabular}{c|c|c} 61.2\% & 68.8\% & 81.1\% \end{tabular}
  & \begin{tabular}{c|c|c} 50.6\% & 59.9\% & 63.1\% \end{tabular}
  & \begin{tabular}{c|c|c} - & - & - \end{tabular}
  & \begin{tabular}{c|c|c} - & - & - \end{tabular}
  & \begin{tabular}{c|c|c} - & - & - \end{tabular} \\
\hline
DenseNet121 
  & \begin{tabular}{c|c|c} 89.6\% & 93.6\% & 95.2\% \end{tabular}
  & \begin{tabular}{c|c|c} 60.4\% & 79.8\% & \textbf{82.1\%} \end{tabular}
  & \begin{tabular}{c|c|c} 48.3\% & 64.0\% & 68.1\% \end{tabular}
  & \begin{tabular}{c|c|c} - & - & - \end{tabular}
  & \begin{tabular}{c|c|c} - & - & - \end{tabular}
  & \begin{tabular}{c|c|c} - & - & - \end{tabular} \\
\hline
\multicolumn{7}{|l|}{\textbf{NAS methods}} \\
\hline
ProxylessNAS 
  & \begin{tabular}{c|c|c} 86.1\% & 89.7\% & 94.1\% \end{tabular}
  & \begin{tabular}{c|c|c} 58.5\% & 78.3\% & 81.1\% \end{tabular}
  & \begin{tabular}{c|c|c} 56.2\% & 63.3\% & 68.6\% \end{tabular}
  & \begin{tabular}{c|c|c} - & - & - \end{tabular}
  & \begin{tabular}{c|c|c} - & - & - \end{tabular}
  & \begin{tabular}{c|c|c} - & - & - \end{tabular} \\
\hline
MNASNet 
  & \begin{tabular}{c|c|c} 76.8\% & 88.0\% & 93.4\% \end{tabular}
  & \begin{tabular}{c|c|c} 45.6\% & 70.4\% & 79.8\% \end{tabular}
  & \begin{tabular}{c|c|c} 53.9\% & 63.2\% & \textbf{69.6\%} \end{tabular}
  & \begin{tabular}{c|c|c} - & - & - \end{tabular}
  & \begin{tabular}{c|c|c} - & - & - \end{tabular}
  & \begin{tabular}{c|c|c} - & - & - \end{tabular} \\
\hline
NASNet 
  & \begin{tabular}{c|c|c} 85.1\% & 92.9\% & 94.9\% \end{tabular}
  & \begin{tabular}{c|c|c} 62.6\% & 77.6\% & 81.9\% \end{tabular}
  & \begin{tabular}{c|c|c} 57.7\% & 64.7\% & 68.6\% \end{tabular}
  & \begin{tabular}{c|c|c} - & - & - \end{tabular}
  & \begin{tabular}{c|c|c} - & - & - \end{tabular}
  & \begin{tabular}{c|c|c} - & - & - \end{tabular} \\
\hline
OFA 
  & \begin{tabular}{c|c|c} - & - & - \end{tabular}
  & \begin{tabular}{c|c|c} - & - & - \end{tabular}
  & \begin{tabular}{c|c|c} - & - & - \end{tabular}
  & \begin{tabular}{c|c|c} - & - & - \end{tabular}
  & \begin{tabular}{c|c|c} - & - & - \end{tabular}
  & \begin{tabular}{c|c|c} - & - & - \end{tabular} \\
\hline
\multicolumn{7}{|l|}{\textbf{MedNNS (ours)}} \\
\hline
MedNNS\textsubscript{T1} 
  & \begin{tabular}{c|c|c} 87.5\% & \textbf{93.6\%} & 94.4\% \end{tabular}
  & \begin{tabular}{c|c|c} \textbf{68.0\%} & 79.4\% & 81.8\% \end{tabular}
  & \begin{tabular}{c|c|c} 57.1\% & 64.5\% & 69.0\% \end{tabular}
  & \begin{tabular}{c|c|c} - & - & - \end{tabular}
  & \begin{tabular}{c|c|c} - & - & - \end{tabular}
  & \begin{tabular}{c|c|c} - & - & - \end{tabular} \\
\hline
MedNNS\textsubscript{T5} 
  & \begin{tabular}{c|c|c} \textbf{91.8\%} & \textbf{93.6\%} & \textbf{96.2\%} \end{tabular}
  & \begin{tabular}{c|c|c} \textbf{74.8\%} & \textbf{80.6\%} & \textbf{82.1\%} \end{tabular}
  & \begin{tabular}{c|c|c} \textbf{58.4\%} & 64.5\% & 69.1\% \end{tabular}
  & \begin{tabular}{c|c|c} - & - & - \end{tabular}
  & \begin{tabular}{c|c|c} - & - & - \end{tabular}
  & \begin{tabular}{c|c|c} - & - & - \end{tabular} \\
\hline
MedNNS\textsubscript{T10} 
  & \begin{tabular}{c|c|c} \textbf{91.8\%} & \textbf{93.8\%} & \textbf{96.2\%} \end{tabular}
  & \begin{tabular}{c|c|c} \textbf{74.8\%} & \textbf{80.6\%} & \textbf{82.4\%} \end{tabular}
  & \begin{tabular}{c|c|c} \textbf{58.4\%} & \textbf{65.0\%} & 69.2\% \end{tabular}
  & \begin{tabular}{c|c|c} - & - & - \end{tabular}
  & \begin{tabular}{c|c|c} - & - & - \end{tabular}
  & \begin{tabular}{c|c|c} - & - & - \end{tabular} \\
\hline
\end{tabular}
\end{adjustbox}
\caption{Comparison of Methods Across Datasets. Each cell lists test accuracies at Epochs 1, 10, and 100 with a vertical line separating the values.}
\label{tab:line_sep_epochs_vert}
\end{table}



\begin{table}[ht]
\centering
\renewcommand{\arraystretch}{1.2}
\begin{adjustbox}{max width=1\textwidth}
\begin{tabular}{|l|c|c|c|c|c|c|}
\hline
\textbf{Method} & \textbf{Pneumonia} & \textbf{OrganS} & \textbf{Tissue} & \textbf{Derma} & \textbf{Blood} & \textbf{Breast} \\
\hline
\multicolumn{7}{|c|}{Test Accuracies: Epoch 1 / Epoch 10 / Epoch 100} \\
\hline
\multicolumn{7}{|l|}{\textbf{Models}} \\
\hline
MobileNetV3 & 85.6\% / 88.5\% / 92.8\% & -\% / -\% / -\% & -\% / -\% / -\% & -\% / -\% / -\% & 73.0\% / 81.0\% / 88.6\% & 28.2\% / 73.7\% / 85.9\% \\
\hline
EfficientNet\textsubscript{B0} & 64.4\% / 85.6\% / 92.3\% & 55.3\% / 78.1\% / 81.2\% & -\% / -\% / -\% & -\% / -\% / -\% & 55.8\% / 75.7\% / 87.2\% & 67.9\% / 77.6\% / 83.3\% \\
\hline
EfficientNet\textsubscript{B4} & 73.1\% / 85.6\% / 92.0\% & 42.2\% / 74.5\% / 81.1\% & -\% / -\% / -\% & 66.9\% / 68.7\% / 74.3\% & 63.3\% / 82.8\% / 96.2\% & 71.2\% / 73.7\% / 87.2\% \\
\hline
ResNet18 & 89.1\% / 93.1\% / 95.2\% & 60.4\% / 66.5\% / 80.6\% & -\% / -\% / -\% & -\% / -\% / -\% & 81.1\% / 91.9\% / 96.2\% & 67.3\% / 85.9\% / 89.7\% \\
\hline
ResNet50 & 81.7\% / 91.3\% / 93.9\% & 61.2\% / 68.8\% / 81.1\% & 50.6\% / 59.9\% / 63.1\% & -\% / -\% / -\% & 79.4\% / 87.3\% / 89.4\% & \textbf{77.6\%} / 79.5\% / 89.1\% \\
\hline
DenseNet121 & 89.6\% / 93.6\% / 95.2\% & 60.4\% / 79.8\% / \textbf{82.1\%} & 48.3\% / 64.0\% / 68.1\% & 70.5\% / 72.9\% / 75.9\% & 83.0\% / 91.6\% / 96.4\% & 67.9\% / 82.0\% / 89.1\% \\
\hline
\multicolumn{7}{|l|}{\textbf{NAS methods}} \\
\hline
ProxylessNAS & 86.1\% / 89.7\% / 94.1\% & 58.5\% / 78.3\% / 81.1\% & 56.2\% / 63.3\% / 68.6\% & 69.2\% / 71.5\% / 76.1\% & 75.5\% / 92.4\% / 96.4\% & 73.0\% / 84.6\% / 89.7\% \\
\hline
MNASNet & 76.8\% / 88.0\% / 93.4\% & 45.6\% / 70.4\% / 79.8\% & 53.9\% / 63.2\% / \textbf{69.6\%} & 67.9\% / 71.5\% / 75.0\% & 56.9\% / 88.0\% / 96.2\% & 37.8\% / 78.8\% / 87.8\% \\
\hline
NASNet & 85.1\% / 92.9\% / 94.9\% & 62.6\% / 77.6\% / 81.9\% & 57.7\% / 64.7\% / 68.6\% & 69.3\% / 71.0\% / 75.4\% & 77.7\% / 91.5\% / 96.0\% & 73.0\% / 83.3\% / 90.4\% \\
\hline
OFA & -\% / -\% / -\% & -\% / -\% / -\% & -\% / -\% / -\% & -\% / -\% / -\% & -\% / -\% / -\% & -\% / -\% / -\% \\
\hline
\multicolumn{7}{|l|}{\textbf{MedNNS (ours)}} \\
\hline
MedNNS\textsubscript{T1} & 87.5\% / \textbf{93.6\%} / 94.4\% & \textbf{68.0\%} / 79.4\% / 81.8\% & 57.1\% / 64.5\% / 69.0\% & \textbf{70.3\%} / \textbf{75.5\%} / \textbf{79.7\%} & \textbf{83.7\%} / \textbf{94.8\%} / \textbf{96.6\%} & 73.0\% / \textbf{86.5\%} / \textbf{92.3\%} \\
\hline
MedNNS\textsubscript{T5} & \textbf{91.8\%} / \textbf{93.6\%} / \textbf{96.2\%} & \textbf{74.8\%} / \textbf{80.6\%} / \textbf{82.1\%} & \textbf{58.4\%} / 64.5\% / 69.1\% & \textbf{70.6\%} / \textbf{76.2\%} / \textbf{79.7\%} & \textbf{86.9\%} / \textbf{95.8\%} / \textbf{97.5\%} & 74.4\% / \textbf{87.2\%} / \textbf{92.3\%} \\
\hline
MedNNS\textsubscript{T10} & \textbf{91.8\%} / \textbf{93.8\%} / \textbf{96.2\%} & \textbf{74.8\%} / \textbf{80.6\%} / \textbf{82.4\%} & \textbf{58.4\%} / \textbf{65.0\%} / 69.2\% & \textbf{70.8\%} / \textbf{77.0\%} / \textbf{79.7\%} & \textbf{86.9\%} / \textbf{95.8\%} / \textbf{97.5\%} & 75.0\% / \textbf{90.4\%} / \textbf{92.3\%} \\
\hline
\end{tabular}
\end{adjustbox}
\caption{Comparison of Methods Across Datasets. Each cell lists test accuracies at Epochs 1, 10, and 100 (in that order).}
\label{tab:compact_no_ep50_random}
\end{table}


\begin{table}[t]
\caption{Comparison of Methods Across Datasets. Each row lists test accuracies at Epoch~10 (@10) and Epoch~100 (@100) to show convergence speed and final accuracy. The final column reports the average across all datasets.}
\label{tab:res}
\centering
% \renewcommand{\arraystretch}{1.2}
\begin{adjustbox}{max width=\textwidth}
\begin{tabular}{|l|cc|cc|cc|cc|cc|cc|cc|}
\hline
\multirow{2}{*}{\textbf{Method}} 
  & \multicolumn{2}{c|}{\textbf{Pneumonia}} 
  & \multicolumn{2}{c|}{\textbf{OrganS}} 
  & \multicolumn{2}{c|}{\textbf{Tissue}} 
  & \multicolumn{2}{c|}{\textbf{Derma}} 
  & \multicolumn{2}{c|}{\textbf{Blood}} 
  & \multicolumn{2}{c|}{\textbf{Breast}} 
  & \multicolumn{2}{c|}{\textbf{Average}} \\
\cline{2-15}
  & \textbf{@10} & \textbf{@100} 
  & \textbf{@10} & \textbf{@100} 
  & \textbf{@10} & \textbf{@100} 
  & \textbf{@10} & \textbf{@100} 
  & \textbf{@10} & \textbf{@100} 
  & \textbf{@10} & \textbf{@100} 
  & \textbf{@10} & \textbf{@100} \\
\hline
\multicolumn{15}{|l|}{\textbf{DL models pretrained with Imagenet}} \\
\hline
MobileNetV3\cite{koonce2021mobilenetv3}     
  & 88.5\% & 92.8\% 
  & 71.3\% & 76.0\%   
  & 58.8\% & 68.1\%   
  & 66.9\% & 75.1\%   
  & 81.0\% & 88.6\% 
  & 73.7\% & 85.9\% 
  & 73.4\% & 81.1\%\\

EfficientNet\textsubscript{B0}\cite{tan2019efficientnet}
  & 85.6\% & 92.3\% 
  & 78.1\% & 81.2\% 
  & 64.4\% & 69.4\%   
  & 70.8\% & 76.2\%   
  & 75.7\% & 87.2\% 
  & 77.6\% & 83.3\% 
  & 75.4\% & 81.6\%\\

EfficientNet\textsubscript{B4}\cite{tan2019efficientnet} 
  & 85.6\% & 92.0\% 
  & 74.5\% & 81.1\% 
  & 55.4\% & 68.7\%   
  & 68.7\% & 74.3\% 
  & 82.8\% & 96.2\% 
  & 73.7\% & 87.2\% 
  & 77.8\% & 83.3\%\\

ResNet18\cite{he2016deep}          
  & 93.1\% & 95.2\% 
  & 66.5\% & 80.6\% 
  & 57.6\% & 66.8\%   
  & 72.0\% & 75.0\%   
  & 91.9\% & 96.2\% 
  & 85.9\% & 89.7\% 
  & 76.5\% & 83.9\%\\

ResNet50\cite{he2016deep}        
  & 91.3\% & 93.9\% 
  & 68.8\% & 81.1\% 
  & 59.9\% & 63.1\% 
  & 72.3\% & 75.0\%   
  & 87.3\% & 92.1\% 
  & 79.5\% & 89.1\% 
  & 80.7\% & 82.4\%\\

DenseNet121\cite{huang2017densely}        
  & 93.6\% & 95.2\% 
  & 79.8\% & 82.1\%
  & 64.0\% & 68.1\% 
  & 72.9\% & 75.9\% 
  & 91.6\% & 96.4\% 
  & 82.0\% & 89.1\% 
  & 80.0\%  & 84.5\%\\
\hline
\multicolumn{15}{|l|}{\textbf{NAS methods}} \\
\hline
ProxylessNAS\cite{cai2018proxylessnas}   
  & 89.7\% & 94.1\% 
  & 78.3\% & 81.1\% 
  & 63.3\% & 68.6\% 
  & 71.5\% & 76.1\% 
  & 92.4\% & 96.4\% 
  & 84.6\% & 89.7\% 
  & 76.7\% & 84.3\% \\

MNASNet\cite{tan2019mnasnet}           
  & 88.0\% & 93.4\% 
  & 70.4\% & 79.8\% 
  & 63.2\% & \textbf{69.6\%} 
  & 71.5\% & 75.0\% 
  & 88.0\% & 96.2\% 
  & 78.8\% & 87.8\% 
  & 80.17\%& 83.6\% \\

NASNet\cite{zoph2018learning}             
  & 92.9\% & 94.9\% 
  & 77.6\% & 81.9\% 
  & 64.7\% & 68.6\% 
  & 71.0\% & 75.4\% 
  & 91.5\% & 96.0\% 
  & 83.3\% & 90.4\% 
  & 80.17\%& 84.5\%\\

PNASNet\cite{liu2018progressive}             
  & 93.1\% & 94.4\% 
  & 75.8\% & 80.8\% 
  & 63.0\% & 69.1\% 
  & 72.8\% & 75.0\% 
  & 93.3\% & 95.9\% 
  & 82.7\% & 87.2\% 
  & 80.12\%& 83.7\% \\

HardcoreNAS\cite{nayman2021hardcore}             
  & 88.3\% & 92.5\% 
  & 71.5\% & 80.9\% 
  & 62.3\% & 68.7\% 
  & 72.0\% & 75.1\% 
  & 84.8\% & 96.3\% 
  & 79.5\% & 85.3\% 
  & 76.4\% & 83.1\%\\

OFA\cite{cai2019once}                
  & 92.2\% & 93.8\%   
  & 66.4\% & 80.1\%   
  & 58.1\% & 67.2\%   
  & 72.2\% & 75.1\%   
  & 90.3\% & 93.4\%   
  & 84.1\% & 89.3\%   
  & 77.2\% & 83.2\%\\
\hline
\multicolumn{15}{|l|}{\textbf{MedNNS (ours)}} \\
\hline
MedNNS\textsubscript{T1} 
  & \textbf{93.6\%} & 94.4\% 
  & 79.4\% & 81.8\% 
  & 64.5\% & 69.0\% 
  & \textbf{75.5\%} & \textbf{79.7\%} 
  & \textbf{94.8\%} & \textbf{96.6\%} 
  & \textbf{86.5\%} & \textbf{92.3\%} 
  & \textbf{82.4\%} & \textbf{85.6\%}\\

MedNNS\textsubscript{T5} 
  & \textbf{93.6\%} & \textbf{96.2\%} 
  & \textbf{80.6\%} & \textbf{82.1\%} 
  & 64.5\% & 69.1\% 
  & \textbf{76.2\%} & \textbf{79.7\%} 
  & \textbf{95.8\%} & \textbf{97.5\%} 
  & \textbf{87.2\%} & \textbf{92.3\%} 
  & \textbf{83.0\%} & \textbf{86.2\%}\\

MedNNS\textsubscript{T10} 
  & \textbf{93.8\%} & \textbf{96.2\%} 
  & \textbf{80.6\%} & \textbf{82.4\%} 
  & \textbf{65.0\%} & 69.2\% 
  & \textbf{77.0\%} & \textbf{79.7\%} 
  & \textbf{95.8\%} & \textbf{97.5\%} 
  & \textbf{90.4\%} & \textbf{92.3\%} 
  & \textbf{83.8\%} & \textbf{86.2\%}\\
\hline
\end{tabular}
\end{adjustbox}
\end{table}

\begin{table}[t]
\caption{Comparison of Methods Across Datasets reporting test accuracies at Epoch~10 (@10) and Epoch~100 (@100) to show convergence speed and final accuracy.}
\label{tab:res}
\centering
\begin{adjustbox}{max width=0.95\textwidth}
\begin{tabular}{lcc | c c| c c |c c |c c |c c |c c}
\toprule
\multirow{2}{*}{\textbf{Method}} 
  & \multicolumn{2}{c}{\textbf{Pneumonia}} 
  & \multicolumn{2}{c}{\textbf{OrganS}} 
  & \multicolumn{2}{c}{\textbf{Tissue}} 
  & \multicolumn{2}{c}{\textbf{Derma}} 
  & \multicolumn{2}{c}{\textbf{Blood}} 
  & \multicolumn{2}{c}{\textbf{Breast}} 
  & \multicolumn{2}{c}{\textbf{Average}} \\
\cmidrule(lr){2-3}\cmidrule(lr){4-5}\cmidrule(lr){6-7}\cmidrule(lr){8-9}\cmidrule(lr){10-11}\cmidrule(lr){12-13}\cmidrule(lr){14-15}
  & \textbf{@10} & \textbf{@100} 
  & \textbf{@10} & \textbf{@100} 
  & \textbf{@10} & \textbf{@100} 
  & \textbf{@10} & \textbf{@100} 
  & \textbf{@10} & \textbf{@100} 
  & \textbf{@10} & \textbf{@100} 
  & \textbf{@10} & \textbf{@100} \\
\midrule
\multicolumn{15}{l}{\textbf{DL models pretrained with Imagenet}} \\
\midrule
MobileNetV3\cite{koonce2021mobilenetv3}     
  & 88.5\% & 92.8\% 
  & 71.3\% & 76.0\%   
  & 58.8\% & 68.1\%   
  & 66.9\% & 75.1\%   
  & 81.0\% & 88.6\% 
  & 73.7\% & 85.9\% 
  & 73.4\% & 81.1\%\\[0.75ex]
EfficientNet\textsubscript{B0}\cite{tan2019efficientnet}
  & 85.6\% & 92.3\% 
  & 78.1\% & 81.2\% 
  & 64.4\% & 69.4\%   
  & 70.8\% & 76.2\%   
  & 75.7\% & 87.2\% 
  & 77.6\% & 83.3\% 
  & 75.4\% & 81.6\%\\[0.75ex]
EfficientNet\textsubscript{B4}\cite{tan2019efficientnet} 
  & 85.6\% & 92.0\% 
  & 74.5\% & 81.1\% 
  & 55.4\% & 68.7\%   
  & 68.7\% & 74.3\% 
  & 82.8\% & 96.2\% 
  & 73.7\% & 87.2\% 
  & 77.8\% & 83.3\%\\[0.75ex]
ResNet18\cite{he2016deep}          
  & 93.1\% & 95.2\% 
  & 66.5\% & 80.6\% 
  & 57.6\% & 66.8\%   
  & 72.0\% & 75.0\%   
  & 91.9\% & 96.2\% 
  & 85.9\% & 89.7\% 
  & 76.5\% & 83.9\%\\[0.75ex]
ResNet50\cite{he2016deep}        
  & 91.3\% & 93.9\% 
  & 68.8\% & 81.1\% 
  & 59.9\% & 63.1\% 
  & 72.3\% & 75.0\%   
  & 87.3\% & 92.1\% 
  & 79.5\% & 89.1\% 
  & 80.7\% & 82.4\%\\[0.75ex]
DenseNet121\cite{huang2017densely}        
  & 93.6\% & 95.2\% 
  & 79.8\% & 82.1\%
  & 64.0\% & 68.1\% 
  & 72.9\% & 75.9\% 
  & 91.6\% & 96.4\% 
  & 82.0\% & 89.1\% 
  & 80.0\% & 84.5\%\\[1ex]
  \hline
\multicolumn{15}{l}{\textbf{NAS methods}} \\
\midrule
ProxylessNAS\cite{cai2018proxylessnas}   
  & 89.7\% & 94.1\% 
  & 78.3\% & 81.1\% 
  & 63.3\% & 68.6\% 
  & 71.5\% & 76.1\% 
  & 92.4\% & 96.4\% 
  & 84.6\% & 89.7\% 
  & 76.7\% & 84.3\% \\[0.75ex]
MNASNet\cite{tan2019mnasnet}           
  & 88.0\% & 93.4\% 
  & 70.4\% & 79.8\% 
  & 63.2\% & \textbf{69.6\%} 
  & 71.5\% & 75.0\% 
  & 88.0\% & 96.2\% 
  & 78.8\% & 87.8\% 
  & 80.17\% & 83.6\% \\[0.75ex]
NASNet\cite{zoph2018learning}             
  & 92.9\% & 94.9\% 
  & 77.6\% & 81.9\% 
  & 64.7\% & 68.6\% 
  & 71.0\% & 75.4\% 
  & 91.5\% & 96.0\% 
  & 83.3\% & 90.4\% 
  & 80.17\% & 84.5\%\\[0.75ex]
PNASNet\cite{liu2018progressive}             
  & 93.1\% & 94.4\% 
  & 75.8\% & 80.8\% 
  & 63.0\% & 69.1\% 
  & 72.8\% & 75.0\% 
  & 93.3\% & 95.9\% 
  & 82.7\% & 87.2\% 
  & 80.12\% & 83.7\% \\[0.75ex]
HardcoreNAS\cite{nayman2021hardcore}             
  & 88.3\% & 92.5\% 
  & 71.5\% & 80.9\% 
  & 62.3\% & 68.7\% 
  & 72.0\% & 75.1\% 
  & 84.8\% & 96.3\% 
  & 79.5\% & 85.3\% 
  & 76.4\% & 83.1\% \\[0.75ex]
OFA\cite{cai2019once}                
  & 92.2\% & 93.8\%   
  & 66.4\% & 80.1\%   
  & 58.1\% & 67.2\%   
  & 72.2\% & 75.1\%   
  & 90.3\% & 93.4\%   
  & 84.1\% & 89.3\%   
  & 77.2\% & 83.2\%\\[1ex]
  \hline
\multicolumn{15}{l}{\textbf{MedNNS (ours)}} \\
\midrule
MedNNS\textsubscript{T1} 
  & \textbf{93.6\%} & 94.4\% 
  & 79.4\% & 81.8\% 
  & 64.5\% & 69.0\% 
  & \textbf{75.5\%} & \textbf{79.7\%} 
  & \textbf{94.8\%} & \textbf{96.6\%} 
  & \textbf{86.5\%} & \textbf{92.3\%} 
  & \textbf{82.4\%} & \textbf{85.6\%}\\[0.75ex]
MedNNS\textsubscript{T5} 
  & \textbf{93.6\%} & \textbf{96.2\%} 
  & \textbf{80.6\%} & \textbf{82.1\%} 
  & 64.5\% & 69.1\% 
  & \textbf{76.2\%} & \textbf{79.7\%} 
  & \textbf{95.8\%} & \textbf{97.5\%} 
  & \textbf{87.2\%} & \textbf{92.3\%} 
  & \textbf{83.0\%} & \textbf{86.2\%}\\[0.75ex]
MedNNS\textsubscript{T10} 
  & \textbf{93.8\%} & \textbf{96.2\%} 
  & \textbf{80.6\%} & \textbf{82.4\%} 
  & \textbf{65.0\%} & 69.2\% 
  & \textbf{77.0\%} & \textbf{79.7\%} 
  & \textbf{95.8\%} & \textbf{97.5\%} 
  & \textbf{90.4\%} & \textbf{92.3\%} 
  & \textbf{83.8\%} & \textbf{86.2\%}\\
\bottomrule
\end{tabular}
\end{adjustbox}

\begin{table}[t]
\caption{Comparison of methods across datasets reporting test accuracies at Epoch~10 (@10) and Epoch~100 (@100) to show convergence speed and final accuracy.}
\label{tab:res}
\centering
\begin{adjustbox}{max width=0.95\textwidth}
\begin{tabular}{c lcc | c c | c c | c c | c c | c c | c c}
\toprule
 & \textbf{Method} 
  & \multicolumn{2}{c}{\textbf{Pneumonia}} 
  & \multicolumn{2}{c}{\textbf{OrganS}} 
  & \multicolumn{2}{c}{\textbf{Tissue}} 
  & \multicolumn{2}{c}{\textbf{Derma}} 
  & \multicolumn{2}{c}{\textbf{Blood}} 
  & \multicolumn{2}{c}{\textbf{Breast}} 
  & \multicolumn{2}{c}{\textbf{Average}} \\
\cmidrule(lr){3-4}\cmidrule(lr){5-6}\cmidrule(lr){7-8}\cmidrule(lr){9-10}\cmidrule(lr){11-12}\cmidrule(lr){13-14}\cmidrule(lr){15-16}
 & 
  & \textbf{@10} & \textbf{@100} 
  & \textbf{@10} & \textbf{@100} 
  & \textbf{@10} & \textbf{@100} 
  & \textbf{@10} & \textbf{@100} 
  & \textbf{@10} & \textbf{@100} 
  & \textbf{@10} & \textbf{@100} 
  & \textbf{@10} & \textbf{@100} \\
\midrule
\multirow{6}{*}{\rotatebox{90}{\textbf{DL models}}} 
 & MobileNetV3\cite{koonce2021mobilenetv3}     
  & 88.5\% & 92.8\% 
  & 71.3\% & 76.0\%   
  & 58.8\% & 68.1\%   
  & 66.9\% & 75.1\%   
  & 81.0\% & 88.6\% 
  & 73.7\% & 85.9\% 
  & 73.4\% & 81.1\%\\[0.75ex]
 & EfficientNet\textsubscript{B0}\cite{tan2019efficientnet}
  & 85.6\% & 92.3\% 
  & 78.1\% & 81.2\% 
  & 64.4\% & 69.4\%   
  & 70.8\% & 76.2\%   
  & 75.7\% & 87.2\% 
  & 77.6\% & 83.3\% 
  & 75.4\% & 81.6\%\\[0.75ex]
 & EfficientNet\textsubscript{B4}\cite{tan2019efficientnet} 
  & 85.6\% & 92.0\% 
  & 74.5\% & 81.1\% 
  & 55.4\% & 68.7\%   
  & 68.7\% & 74.3\% 
  & 82.8\% & 96.2\% 
  & 73.7\% & 87.2\% 
  & 77.8\% & 83.3\%\\[0.75ex]
 & ResNet18\cite{he2016deep}          
  & 93.1\% & 95.2\% 
  & 66.5\% & 80.6\% 
  & 57.6\% & 66.8\%   
  & 72.0\% & 75.0\%   
  & 91.9\% & 96.2\% 
  & 85.9\% & 89.7\% 
  & 76.5\% & 83.9\%\\[0.75ex]
 & ResNet50\cite{he2016deep}        
  & 91.3\% & 93.9\% 
  & 68.8\% & 81.1\% 
  & 59.9\% & 63.1\% 
  & 72.3\% & 75.0\%   
  & 87.3\% & 92.1\% 
  & 79.5\% & 89.1\% 
  & 80.7\% & 82.4\%\\[0.75ex]
 & DenseNet121\cite{huang2017densely}        
  & 93.6\% & 95.2\% 
  & 79.8\% & 82.1\%
  & 64.0\% & 68.1\% 
  & 72.9\% & 75.9\% 
  & 91.6\% & 96.4\% 
  & 82.0\% & 89.1\% 
  & 80.0\% & 84.5\%\\[1ex]
\midrule
\multirow{6}{*}{\rotatebox{90}{\textbf{NAS methods}}} 
 & ProxylessNAS\cite{cai2018proxylessnas}   
  & 89.7\% & 94.1\% 
  & 78.3\% & 81.1\% 
  & 63.3\% & 68.6\% 
  & 71.5\% & 76.1\% 
  & 92.4\% & 96.4\% 
  & 84.6\% & 89.7\% 
  & 76.7\% & 84.3\%\\[0.75ex]
 & MNASNet\cite{tan2019mnasnet}           
  & 88.0\% & 93.4\% 
  & 70.4\% & 79.8\% 
  & 63.2\% & \cellcolor{SkyBlue!20}\textbf{69.6\%} 
  & 71.5\% & 75.0\% 
  & 88.0\% & 96.2\% 
  & 78.8\% & 87.8\% 
  & 80.17\% & 83.6\%\\[0.75ex]
 & NASNet\cite{zoph2018learning}             
  & 92.9\% & 94.9\% 
  & 77.6\% & 81.9\% 
  & 64.7\% & 68.6\% 
  & 71.0\% & 75.4\% 
  & 91.5\% & 96.0\% 
  & 83.3\% & 90.4\% 
  & 80.17\% & 84.5\%\\[0.75ex]
 & PNASNet\cite{liu2018progressive}             
  & 93.1\% & 94.4\% 
  & 75.8\% & 80.8\% 
  & 63.0\% & 69.1\% 
  & 72.8\% & 75.0\% 
  & 93.3\% & 95.9\% 
  & 82.7\% & 87.2\% 
  & 80.12\% & 83.7\%\\[0.75ex]
 & HardcoreNAS\cite{nayman2021hardcore}             
  & 88.3\% & 92.5\% 
  & 71.5\% & 80.9\% 
  & 62.3\% & 68.7\% 
  & 72.0\% & 75.1\% 
  & 84.8\% & 96.3\% 
  & 79.5\% & 85.3\% 
  & 76.4\% & 83.1\%\\[0.75ex]
 & OFA\cite{cai2019once}                
  & 92.2\% & 93.8\%   
  & 66.4\% & 80.1\%   
  & 58.1\% & 67.2\%   
  & 72.2\% & 75.1\%   
  & 90.3\% & 93.4\%   
  & 84.1\% & 89.3\%   
  & 77.2\% & 83.2\%\\[1ex]
\midrule
\multirow{3}{*}{\rotatebox{90}{\textbf{MedNNS (ours)}}} 
 & MedNNS\textsubscript{T1} 
  & \cellcolor{SkyBlue!20}\textbf{93.6\%} & 94.4\% 
  & 79.4\% & 81.8\% 
  & 64.5\% & 69.0\% 
  & \cellcolor{SkyBlue!20}\textbf{75.5\%} & \cellcolor{SkyBlue!20}\textbf{79.7\%} 
  & \cellcolor{SkyBlue!20}\textbf{94.8\%} & \cellcolor{SkyBlue!20}\textbf{96.6\%} 
  & \cellcolor{SkyBlue!20}\textbf{86.5\%} & \cellcolor{SkyBlue!20}\textbf{92.3\%} 
  & \cellcolor{SkyBlue!20}\textbf{82.4\%} & \cellcolor{SkyBlue!20}\textbf{85.6\%}\\[0.75ex]
 & MedNNS\textsubscript{T5} 
  & \cellcolor{SkyBlue!20}\textbf{93.6\%} & \cellcolor{SkyBlue!20}\textbf{96.2\%} 
  & \cellcolor{SkyBlue!20}\textbf{80.6\%} & \cellcolor{SkyBlue!20}\textbf{82.1\%} 
  & 64.5\% & 69.1\% 
  & \cellcolor{SkyBlue!20}\textbf{76.2\%} & \cellcolor{SkyBlue!20}\textbf{79.7\%} 
  & \cellcolor{SkyBlue!20}\textbf{95.8\%} & \cellcolor{SkyBlue!20}\textbf{97.5\%} 
  & \cellcolor{SkyBlue!20}\textbf{87.2\%} & \cellcolor{SkyBlue!20}\textbf{92.3\%} 
  & \cellcolor{SkyBlue!20}\textbf{83.0\%} & \cellcolor{SkyBlue!20}\textbf{86.2\%}\\[0.75ex]
 & MedNNS\textsubscript{T10} 
  & \cellcolor{SkyBlue!20}\textbf{93.8\%} & \cellcolor{SkyBlue!20}\textbf{96.2\%} 
  & \cellcolor{SkyBlue!20}\textbf{80.6\%} & \cellcolor{SkyBlue!20}\textbf{82.4\%} 
  & \cellcolor{SkyBlue!20}\textbf{65.0\%} & 69.2\% 
  & \cellcolor{SkyBlue!20}\textbf{77.0\%} & \cellcolor{SkyBlue!20}\textbf{79.7\%} 
  & \cellcolor{SkyBlue!20}\textbf{95.8\%} & \cellcolor{SkyBlue!20}\textbf{97.5\%} 
  & \cellcolor{SkyBlue!20}\textbf{90.4\%} & \cellcolor{SkyBlue!20}\textbf{92.3\%} 
  & \cellcolor{SkyBlue!20}\textbf{83.8\%} & \cellcolor{SkyBlue!20}\textbf{86.2\%}\\
\bottomrule
\end{tabular}
\end{adjustbox}
\end{table}

